Recognising Cardiac Abnormalities in Wearable Device Photoplethysmography (PPG) with Deep Learning

Cardiac abnormalities affecting heart rate and rhythm are commonly observed in both healthy and acutely unwell people. Although many of these are benign, they can sometimes indicate a serious health risk. ECG monitors are typically used to detect these events in electrical heart activity, however they are impractical for continuous long-term use. In contrast, current-generation wearables with optical photoplethysmography (PPG) have gained popularity with their low-cost, lack of wires and tiny size. Many cardiac abnormalities such as ectopic beats and AF can manifest as both obvious and subtle anomalies in a PPG waveform as they disrupt blood flow. We propose an automatic method for recognising these anomalies in PPG signal alone, without the need for ECG. We train an LSTM deep neural network on 400,000 clean PPG samples to learn typical PPG morphology and rhythm, and flag PPG signal diverging from this as cardiac abnormalities. We compare the cardiac abnormalities our approach recognises with the ectopic beats recorded by a bedside ECG monitor for 29 patients over 47.6 hours of gold standard observations. Our proposed cardiac abnormality recognition approach recognises 60%+ of ECG-detected PVCs in PPG signal, with a false positive rate of 23% - demonstrating the compelling power and value of this novel approach. Finally we examine how cardiac abnormalities manifest in PPG signal for in- and out-of-hospital patient populations using a wearable device during standard care.

==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

